Interim recommendations for the evaluation of Higgs production cross sections and branching ratios at the LHC in the Two-Higgs-Doublet Model

In this note we give interim recommendations on how to evaluate LHC cross sections for (neutral) Higgs production and Higgs branching ratios in the general (CP-conserving) Two-Higgs-Doublet Model (2HDM). The current status of available higher-order corrections to Higgs production and decay in this model is discussed, and the existing public codes implementing these calculations are described. Numerical results are presented for a set of reference scenarios, demonstrating the very good agreement between the results obtained using different programs.

==> tables/noew/table-ggh-A.tex <==
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline$\sqrt{s}$ & \multicolumn{3}{|c|}{$\sigma(gg\to h)$/pb} &\multicolumn{3}{|c|}{ $\sigma(gg\to H)$/pb} &\multicolumn{3}{|c|}{ $\sigma(gg\to A)$/pb} \\
  /TeV &{\tt SusHi} & {\tt HIGLU} & $\%$ &{\tt SusHi} & {\tt HIGLU} & $\%$ &{\tt SusHi} & {\tt HIGLU} & $\%$ \\\hline
$ 7$ & $  21.24$ & $  21.25$ & $  0.0$ & $  0.06995$ & $  0.06996$ & $  0.0$ & $  4.061$ & $  4.063$ & $  0.06$\\ 
 $ 8$ & $  27.07$ & $  27.07$ & $  0.0$ & $  0.09615$ & $  0.09617$ & $  0.0$ & $  5.639$ & $  5.642$ & $  0.06$\\ 
 $ 13$ & $  61.77$ & $  61.79$ & $  0.0$ & $  0.2765$ & $  0.2766$ & $  0.1$ & $  16.69$ & $  16.70$ & $  0.06$\\ 
 $ 14$ & $  69.59$ & $  69.60$ & $  0.0$ & $  0.3210$ & $  0.3212$ & $  0.1$ & $  19.45$ & $  19.46$ & $  0.06$\\ 
 \hline
\end{tabular}


==> tables/noew/table-ggh-B.tex <==
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline$\sqrt{s}$ & \multicolumn{3}{|c|}{$\sigma(gg\to h)$/pb} &\multicolumn{3}{|c|}{ $\sigma(gg\to H)$/pb} &\multicolumn{3}{|c|}{ $\sigma(gg\to A)$/pb} \\
  /TeV &{\tt SusHi} & {\tt HIGLU} & $\%$ &{\tt SusHi} & {\tt HIGLU} & $\%$ &{\tt SusHi} & {\tt HIGLU} & $\%$ \\\hline
$ 7$ & $  17.22$ & $  17.22$ & $  0.0$ & $  2.024$ & $  2.023$ & $  0.0$ & $  3.979$ & $  3.978$ & $  0.02$\\ 
 $ 8$ & $  21.87$ & $  21.88$ & $  0.0$ & $  2.756$ & $  2.756$ & $  0.0$ & $  5.355$ & $  5.354$ & $  0.01$\\ 
 $ 13$ & $  49.39$ & $  49.40$ & $  0.0$ & $  7.653$ & $  7.652$ & $  0.0$ & $  14.34$ & $  14.34$ & $  0.03$\\ 
 $ 14$ & $  55.55$ & $  55.56$ & $  0.0$ & $  8.837$ & $  8.835$ & $  0.0$ & $  16.49$ & $  16.48$ & $  0.03$\\ 
 \hline
\end{tabular}


==> tables/noew/table-ggh-C.tex <==
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline$\sqrt{s}$ & \multicolumn{3}{|c|}{$\sigma(gg\to h)$/pb} &\multicolumn{3}{|c|}{ $\sigma(gg\to H)$/pb} &\multicolumn{3}{|c|}{ $\sigma(gg\to A)$/pb} \\
  /TeV &{\tt SusHi} & {\tt HIGLU} & $\%$ &{\tt SusHi} & {\tt HIGLU} & $\%$ &{\tt SusHi} & {\tt HIGLU} & $\%$ \\\hline
$ 7$ & $  15.46$ & $  15.47$ & $  0.0$ & $  0.02702$ & $  0.02702$ & $  0.0$ & $  0.02421$ & $  0.02422$ & $  0.06$\\ 
 $ 8$ & $  19.69$ & $  19.70$ & $  0.0$ & $  0.03814$ & $  0.03814$ & $  0.0$ & $  0.03575$ & $  0.03576$ & $  0.04$\\ 
 $ 13$ & $  44.85$ & $  44.86$ & $  0.0$ & $  0.1177$ & $  0.1177$ & $  0.0$ & $  0.1269$ & $  0.1269$ & $  0.02$\\ 
 $ 14$ & $  50.51$ & $  50.52$ & $  0.0$ & $  0.1377$ & $  0.1377$ & $  0.0$ & $  0.1513$ & $  0.1514$ & $  0.08$\\ 
 \hline
\end{tabular}

